Perceptual Artifacts Localization for Inpainting

Image inpainting is an essential task for multiple practical applications like object removal and image editing. Deep GAN-based models greatly improve the inpainting performance in structures and textures within the hole, but might also generate unexpected artifacts like broken structures or color blobs. Users perceive these artifacts to judge the effectiveness of inpainting models, and retouch these imperfect areas to inpaint again in a typical retouching workflow. Inspired by this workflow, we propose a new learning task of automatic segmentation of inpainting perceptual artifacts, and apply the model for inpainting model evaluation and iterative refinement. Specifically, we first construct a new inpainting artifacts dataset by manually annotating perceptual artifacts in the results of state-of-the-art inpainting models. Then we train advanced segmentation networks on this dataset to reliably localize inpainting artifacts within inpainted images. Second, we propose a new interpretable evaluation metric called Perceptual Artifact Ratio (PAR), which is the ratio of objectionable inpainted regions to the entire inpainted area. PAR demonstrates a strong correlation with real user preference. Finally, we further apply the generated masks for iterative image inpainting by combining our approach with multiple recent inpainting methods. Extensive experiments demonstrate the consistent decrease of artifact regions and inpainting quality improvement across the different methods.

==> tables/iterative_fill.tex <==
\begin{table*}[h!]
    \begin{center}
     \resizebox{\textwidth}{!}{
      \begin{tabular}
      {c|c|c|c|c|c|c}
        \toprule % <-- Toprule here
        \hspace{10pt} \textbf{Models} \hspace{10pt} & \ \hspace{0pt} Original Fill \hspace{0pt} & \ \hspace{5pt} $1^{st}$ ReFill \hspace{5pt} & \ \hspace{5pt} $2^{nd}$ ReFill \hspace{5pt} & \ \hspace{5pt} $3^{rd}$ ReFill \hspace{5pt} & \ \hspace{5pt} $4^{th}$ ReFill \hspace{5pt} & \ \hspace{5pt} $5^{th}$ ReFill \hspace{5pt} \\
        \midrule % <-- Midrule here
        LaMa & 0.3789 & 0.2439 (-35.63\%) & 0.1811 (-25.75\%) & 0.1464 (-19.16\%) & 0.1241 (-15.23\%) & 0.1091 (-12.09\%) \\
        \midrule % <-- Midrule here
        ProFill & 0.3809 & 0.3249 (-14.70\%) & 0.2945 (-9.33\%) & 0.2749 (-6.69\%) & 0.2586 (-5.92\%) & 0.2442 (-5.57\%) \\
        \midrule % <-- Midrule here
        CoMod-GAN & 0.4912 & 0.4314 (-12.17\%) & 0.3976 (-7.83\%) & 0.3715 (-6.56\%) & 0.3521 (-5.22\%) & 0.3370 (-4.29\%)   \\
        \midrule % <-- Midrule here
        EdgeConnect & 0.4975 & 0.4340 (-12.76\%) & 0.4095 (-5.64\%) & 0.3918 (-4.32\%) & 0.3763 (-3.96\%) & 0.3673 (-2.39\%)  \\
        % \midrule % <-- Midrule here
        % DeepFillv2 & 0.1644 & 0.09776 & 0.8952 & 0.9418 & 0.0986 & 0.0986   \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      }
      \vspace{5 pt}
      \caption{The detected bad filled regions over iterations of refill. The reported numbers represent the averaged ratio of predicted bad filled area over the hole mask area. }
      \label{tab:iterative_fill}
    \end{center}
    \vspace{-15 pt}
\end{table*}






